Variable resolution Poisson-disk sampling for meshing discrete fracture networks

We present the near-Maximal Algorithm for Poisson-disk Sampling (nMAPS) to generate point distributions for variable resolution Delaunay triangular and tetrahedral meshes in two and three-dimensions, respectively. nMAPS consists of two principal stages. In the first stage, an initial point distribution is produced using a cell-based rejection algorithm. In the second stage, holes in the sample are detected using an efficient background grid and filled in to obtain a near-maximal covering. Extensive testing shows that nMAPS generates a variable resolution mesh in linear run time with the number of accepted points. We demonstrate nMAPS capabilities by meshing three-dimensional discrete fracture networks (DFN) and the surrounding volume. The discretized boundaries of the fractures, which are represented as planar polygons, are used as the seed of 2D-nMAPS to produce a conforming Delaunay triangulation. The combined mesh of the DFN is used as the seed for 3D-nMAPS, which produces conforming Delaunay tetrahedra surrounding the network. Under a set of conditions that naturally arise in maximal Poisson-disk samples and are satisfied by nMAPS, the two-dimensional Delaunay triangulations are guaranteed to only have well-behaved triangular faces. While nMAPS does not provide triangulation quality bounds in more than two dimensions, we found that low-quality tetrahedra in 3D are infrequent, can be readily detected and removed, and a high quality balanced mesh is produced.

==> graphics/plots/bench_k_part2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1210,704){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(1210,1356){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1210,2007){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(1210,2659){\makebox(0,0)[r]{\strut{}$100000$}}%
      \put(1740,484){\makebox(0,0){\strut{}$10$}}%
      \put(2741,484){\makebox(0,0){\strut{}$100$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}no. of nodes}}}%
      \put(2493,154){\makebox(0,0){\strut{}k}}%
      \csname LTb\endcsname%%
      \put(3949,704){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3949,1041){\makebox(0,0)[l]{\strut{}$1$}}%
      \put(3949,1378){\makebox(0,0)[l]{\strut{}$2$}}%
      \put(3949,1715){\makebox(0,0)[l]{\strut{}$3$}}%
      \put(3949,2052){\makebox(0,0)[l]{\strut{}$4$}}%
      \put(3949,2389){\makebox(0,0)[l]{\strut{}$5$}}%
      \put(4147,1681){\rotatebox{-270}{\makebox(0,0){\strut{}repetitions}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_k_part2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphics/plots/bench_k_time1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,901){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \put(682,1293){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,1686){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(682,2079){\makebox(0,0)[r]{\strut{}$10^2$}}%
      \put(682,2471){\makebox(0,0)[r]{\strut{}$10^3$}}%
      \put(814,484){\makebox(0,0){\strut{}$10^{0.5}$}}%
      \put(1369,484){\makebox(0,0){\strut{}$10$}}%
      \put(1925,484){\makebox(0,0){\strut{}$10^{1.5}$}}%
      \put(2480,484){\makebox(0,0){\strut{}$10^2$}}%
      \put(3036,484){\makebox(0,0){\strut{}$10^{2.5}$}}%
      \put(3591,484){\makebox(0,0){\strut{}$10^3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}run time [s]}}}%
      \put(2202,154){\makebox(0,0){\strut{}k}}%
      \csname LTb\endcsname%%
      \put(3930,704){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3930,983){\makebox(0,0)[l]{\strut{}$10000$}}%
      \put(3930,1262){\makebox(0,0)[l]{\strut{}$20000$}}%
      \put(3930,1541){\makebox(0,0)[l]{\strut{}$30000$}}%
      \put(3930,1821){\makebox(0,0)[l]{\strut{}$40000$}}%
      \put(3930,2100){\makebox(0,0)[l]{\strut{}$50000$}}%
      \put(3930,2379){\makebox(0,0)[l]{\strut{}$60000$}}%
      \put(3930,2659){\makebox(0,0)[l]{\strut{}$70000$}}%
      \put(4656,1681){\rotatebox{-270}{\makebox(0,0){\strut{}no. of nodes}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_k_time1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/bench_ang.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,704){\makebox(0,0)[r]{\strut{}$18$}}%
      \put(682,921){\makebox(0,0)[r]{\strut{}$19$}}%
      \put(682,1138){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(682,1356){\makebox(0,0)[r]{\strut{}$21$}}%
      \put(682,1573){\makebox(0,0)[r]{\strut{}$22$}}%
      \put(682,1790){\makebox(0,0)[r]{\strut{}$23$}}%
      \put(682,2007){\makebox(0,0)[r]{\strut{}$24$}}%
      \put(682,2225){\makebox(0,0)[r]{\strut{}$25$}}%
      \put(682,2442){\makebox(0,0)[r]{\strut{}$26$}}%
      \put(682,2659){\makebox(0,0)[r]{\strut{}$27$}}%
      \put(931,484){\makebox(0,0){\strut{}$5$}}%
      \put(1294,484){\makebox(0,0){\strut{}$10$}}%
      \put(1658,484){\makebox(0,0){\strut{}$20$}}%
      \put(2021,484){\makebox(0,0){\strut{}$40$}}%
      \put(2384,484){\makebox(0,0){\strut{}$80$}}%
      \put(2747,484){\makebox(0,0){\strut{}$160$}}%
      \put(3111,484){\makebox(0,0){\strut{}$320$}}%
      \put(3474,484){\makebox(0,0){\strut{}$640$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}min. angle [$^\circ$]}}}%
      \put(2202,154){\makebox(0,0){\strut{}k}}%
      \csname LTb\endcsname%%
      \put(3930,704){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3930,1041){\makebox(0,0)[l]{\strut{}$1$}}%
      \put(3930,1378){\makebox(0,0)[l]{\strut{}$2$}}%
      \put(3930,1715){\makebox(0,0)[l]{\strut{}$3$}}%
      \put(3930,2052){\makebox(0,0)[l]{\strut{}$4$}}%
      \put(3930,2389){\makebox(0,0)[l]{\strut{}$5$}}%
      \put(4128,1681){\rotatebox{-270}{\makebox(0,0){\strut{}repetitions}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_ang}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/bench_k_part.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$18000$}}%
      \put(1078,1095){\makebox(0,0)[r]{\strut{}$20000$}}%
      \put(1078,1486){\makebox(0,0)[r]{\strut{}$22000$}}%
      \put(1078,1877){\makebox(0,0)[r]{\strut{}$24000$}}%
      \put(1078,2268){\makebox(0,0)[r]{\strut{}$26000$}}%
      \put(1078,2659){\makebox(0,0)[r]{\strut{}$28000$}}%
      \put(1312,484){\makebox(0,0){\strut{}$5$}}%
      \put(1629,484){\makebox(0,0){\strut{}$10$}}%
      \put(1945,484){\makebox(0,0){\strut{}$20$}}%
      \put(2262,484){\makebox(0,0){\strut{}$40$}}%
      \put(2579,484){\makebox(0,0){\strut{}$80$}}%
      \put(2896,484){\makebox(0,0){\strut{}$160$}}%
      \put(3212,484){\makebox(0,0){\strut{}$320$}}%
      \put(3529,484){\makebox(0,0){\strut{}$640$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}no. of nodes}}}%
      \put(2420,154){\makebox(0,0){\strut{}k}}%
      \csname LTb\endcsname%%
      \put(3945,704){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3945,1041){\makebox(0,0)[l]{\strut{}$1$}}%
      \put(3945,1378){\makebox(0,0)[l]{\strut{}$2$}}%
      \put(3945,1715){\makebox(0,0)[l]{\strut{}$3$}}%
      \put(3945,2052){\makebox(0,0)[l]{\strut{}$4$}}%
      \put(3945,2389){\makebox(0,0)[l]{\strut{}$5$}}%
      \put(4143,1681){\rotatebox{-270}{\makebox(0,0){\strut{}repetitions}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_k_part}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/bench_k_part2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1210,704){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(1210,1356){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(1210,2007){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(1210,2659){\makebox(0,0)[r]{\strut{}$100000$}}%
      \put(1740,484){\makebox(0,0){\strut{}$10$}}%
      \put(2741,484){\makebox(0,0){\strut{}$100$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}no. of nodes}}}%
      \put(2493,154){\makebox(0,0){\strut{}k}}%
      \csname LTb\endcsname%%
      \put(3949,704){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3949,1041){\makebox(0,0)[l]{\strut{}$1$}}%
      \put(3949,1378){\makebox(0,0)[l]{\strut{}$2$}}%
      \put(3949,1715){\makebox(0,0)[l]{\strut{}$3$}}%
      \put(3949,2052){\makebox(0,0)[l]{\strut{}$4$}}%
      \put(3949,2389){\makebox(0,0)[l]{\strut{}$5$}}%
      \put(4147,1681){\rotatebox{-270}{\makebox(0,0){\strut{}repetitions}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_k_part2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/bench_k_time1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,901){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \put(682,1293){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,1686){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(682,2079){\makebox(0,0)[r]{\strut{}$10^2$}}%
      \put(682,2471){\makebox(0,0)[r]{\strut{}$10^3$}}%
      \put(814,484){\makebox(0,0){\strut{}$10^{0.5}$}}%
      \put(1369,484){\makebox(0,0){\strut{}$10$}}%
      \put(1925,484){\makebox(0,0){\strut{}$10^{1.5}$}}%
      \put(2480,484){\makebox(0,0){\strut{}$10^2$}}%
      \put(3036,484){\makebox(0,0){\strut{}$10^{2.5}$}}%
      \put(3591,484){\makebox(0,0){\strut{}$10^3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}run time [s]}}}%
      \put(2202,154){\makebox(0,0){\strut{}k}}%
      \csname LTb\endcsname%%
      \put(3930,704){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3930,983){\makebox(0,0)[l]{\strut{}$10000$}}%
      \put(3930,1262){\makebox(0,0)[l]{\strut{}$20000$}}%
      \put(3930,1541){\makebox(0,0)[l]{\strut{}$30000$}}%
      \put(3930,1821){\makebox(0,0)[l]{\strut{}$40000$}}%
      \put(3930,2100){\makebox(0,0)[l]{\strut{}$50000$}}%
      \put(3930,2379){\makebox(0,0)[l]{\strut{}$60000$}}%
      \put(3930,2659){\makebox(0,0)[l]{\strut{}$70000$}}%
      \put(4656,1681){\rotatebox{-270}{\makebox(0,0){\strut{}no. of nodes}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_k_time1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/bench_k_time2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \put(946,1095){\makebox(0,0)[r]{\strut{}}}%$-3.5$}}%
      \put(946,1486){\makebox(0,0)[r]{\strut{}$10^{-3}$}}%
      \put(946,1877){\makebox(0,0)[r]{\strut{}}}%$-2.5$}}%
      \put(946,2268){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(946,2659){\makebox(0,0)[r]{\strut{}}}%$-1.5$}}%
      \put(1078,484){\makebox(0,0){\strut{}}}%$0.5$}}%
      \put(1586,484){\makebox(0,0){\strut{}$10$}}%
      \put(2094,484){\makebox(0,0){\strut{}}}%$10^{1.5}$}}%
      \put(2602,484){\makebox(0,0){\strut{}$10^2$}}%
      \put(3110,484){\makebox(0,0){\strut{}}}%$10^{2.5}$}}%
      \put(3618,484){\makebox(0,0){\strut{}$10^3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}run time [s]}}}%
      \put(2348,154){\makebox(0,0){\strut{}k}}%
      \csname LTb\endcsname%%
      \put(3941,704){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3941,983){\makebox(0,0)[l]{\strut{}$10000$}}%
      \put(3941,1262){\makebox(0,0)[l]{\strut{}$20000$}}%
      \put(3941,1541){\makebox(0,0)[l]{\strut{}$30000$}}%
      \put(3941,1821){\makebox(0,0)[l]{\strut{}$40000$}}%
      \put(3941,2100){\makebox(0,0)[l]{\strut{}$50000$}}%
      \put(3941,2379){\makebox(0,0)[l]{\strut{}$60000$}}%
      \put(3941,2659){\makebox(0,0)[l]{\strut{}$70000$}}%
      \put(4667,1681){\rotatebox{-270}{\makebox(0,0){\strut{}no. of nodes}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_k_time2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/bench_part_time1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,828){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(682,1270){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,1713){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(682,2155){\makebox(0,0)[r]{\strut{}$10^2$}}%
      \put(682,2597){\makebox(0,0)[r]{\strut{}$10^3$}}%
      \put(814,484){\makebox(0,0){\strut{}$10^{2.5}$}}%
      \put(1369,484){\makebox(0,0){\strut{}$10^{3}$}}%
      \put(1925,484){\makebox(0,0){\strut{}$10^{3.5}$}}%
      \put(2480,484){\makebox(0,0){\strut{}$10^{4}$}}%
      \put(3036,484){\makebox(0,0){\strut{}$10^{4.5}$}}%
      \put(3591,484){\makebox(0,0){\strut{}$10^5$}}%
%      \colorrgb{0.20,0.00,0.25}%%
%      \put(33322037,5693){\makebox(0,0){\strut{}k=5}}%
%      \colorrgb{0.41,0.00,0.86}%%
%      \put(33488657,16749){\makebox(0,0){\strut{}k=10}}%
%      \colorrgb{0.54,0.02,0.97}%%
%      \put(20547837,16749){\rotatebox{8}{\makebox(0,0){\strut{}k=20}}}%
%      \colorrgb{0.65,0.07,0.50}%%
%      \put(19992437,30017){\rotatebox{14}{\makebox(0,0){\strut{}k=40}}}%
%      \colorrgb{0.74,0.16,0.00}%%
%      \put(18326237,54341){\rotatebox{27}{\makebox(0,0){\strut{}k=80}}}%
%      \colorrgb{0.82,0.30,0.00}%%
%      \put(16660037,83088){\rotatebox{41}{\makebox(0,0){\strut{}k=160}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}run time [s]}}}%
      \put(2202,154){\makebox(0,0){\strut{}no. of nodes}}%
      \csname LTb\endcsname%%
      \put(3930,783){\makebox(0,0)[l]{\strut{}$5$}}%
      \put(3930,1028){\makebox(0,0)[l]{\strut{}$10$}}%
      \put(3930,1273){\makebox(0,0)[l]{\strut{}$20$}}%
      \put(3930,1519){\makebox(0,0)[l]{\strut{}$40$}}%
      \put(3930,1764){\makebox(0,0)[l]{\strut{}$80$}}%
      \put(3930,2010){\makebox(0,0)[l]{\strut{}$160$}}%
      \put(3930,2255){\makebox(0,0)[l]{\strut{}$320$}}%
      \put(4392,1681){\rotatebox{-270}{\makebox(0,0){\strut{}k}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_part_time1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/bench_part_time2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(550,1203){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(550,1791){\makebox(0,0)[r]{\strut{}$10$}}%
      \put(550,2380){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(682,484){\makebox(0,0){\strut{}$10^{2.5}$}}%
      \put(1406,484){\makebox(0,0){\strut{}$10^{3}$}}%
      \put(2130,484){\makebox(0,0){\strut{}$10^{3.5}$}}%
      \put(2854,484){\makebox(0,0){\strut{}$10^{4}$}}%
      \put(3578,484){\makebox(0,0){\strut{}$10^{4.5}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,1681){\rotatebox{-270}{\makebox(0,0){\strut{}run time [s]}}}%
      \put(2130,154){\makebox(0,0){\strut{}no. of nodes}}%
      \csname LTb\endcsname%%
      \put(3926,815){\makebox(0,0)[l]{\strut{}$5$}}%
      \put(3926,1161){\makebox(0,0)[l]{\strut{}$10$}}%
      \put(3926,1508){\makebox(0,0)[l]{\strut{}$20$}}%
      \put(3926,1854){\makebox(0,0)[l]{\strut{}$40$}}%
      \put(3926,2201){\makebox(0,0)[l]{\strut{}$80$}}%
      \put(3926,2547){\makebox(0,0)[l]{\strut{}$160$}}%
      \put(4388,1681){\rotatebox{-270}{\makebox(0,0){\strut{}k}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./pics/plots/bench_part_time2}}%
    \gplfronttext
  \end{picture}%
\endgroup

